Bellman functions on simple non-convex domains in the plane

The present paper provides a generalization of the previous authors' work on Bellman functions for integral functionals on $\mathrm{BMO}$. Those Bellman functions are the minimal locally concave functions on parabolic strips in the plane. Now we describe the algorithm for constructing minimal locally concave functions on a planar domain that is a difference of two unbounded convex domains. This leads to many sharp estimates for functions in the classes like $\mathrm{BMO}$, $A_p$, or the Gehring classes.

==> 6Chapter_text.tex <==
\chapter{Related questions and further development}

\section{Related questions}\label{s61}
\subsection{Analytic properties}\label{s611}
In Subsection~\ref{s443}, we proved that there is only a finite number of essential critical points of the evolution. However, this may seem a bit ``unfair'', because these critical point  are only those moments~$\eps$ at which~$\GammaFixed$ changes (see the beginning of Section~\ref{s44} and the proof of Theorem~\ref{BC}). We have not proved that there is only a finite number of moments~$\eps$ where~$\GammaFree$ changes when~$\eps$ belongs to an interval. In particular, it is interesting whether the pattern stabilizes as~$\eps \searrow \eps'$ in Proposition~\ref{MultibirdieDesintegrationSt}. Informally, does a birdie or a multibirdie choose one of many possible ways to desintegrate? %We believe that the answer is ``no'', however, we are not able to construct a counterexample (see Conjecture~\ref{BirdieOscCConj}). 
In general, the answer is ``no'', see the second example in Section~\ref{s54} (this emphasizes that the difficulties we had to overcome in Proposition~\ref{MultibirdieDesintegrationSt} had their origin in the nature of the evolution, not in the authors' heads).

The answer is ``yes'' if one assumes that~$f$ is piecewise analytic. Then, the algorithm is finite in the sense that the graph~$\Gamma(\eps)$ changes only a finite number of times when~$\eps \in (0,\eps_{\infty})$. Indeed, if~$f$ is piecewise analytic, then all the functions~$a$ and~$b$ associated with chordal domains are piecewise analytic (by the implicit function theorem). Thus, the forces are piecewise analytic as functions of~$u$. So, the roots of balance equations are also piecewise analytic as functions of~$\eps$ (again, by the implicit function theorem). Therefore, the graph~$\Gamma(\eps)$ changes only a finite number of times, since each such critical point is a root of an equation between several piecewise analytic functions (and there are only finite number of them). We do not mark this reasoning as a proof, because the precise statement and a rigorous reasoning will take much place. As the reader have seen, in all the examples, the picture stabilizes in a reasonably small number of steps (the only known example where there are many such steps is the one considered in~\cite{CrazySine}, but it was designed to illustrate as many evolutional scenarios as possible).

However, there is a small hope that the behavior of angles (birdies and multibirdies as well) is much ``smoother'' than one can conjecture from the first sight. The proposition below deals with the easiest case of a lonely angle surrounded by tangent domains that last to infinity. We show that such an angle cannot oscillate near a point.

\begin{St}\label{AnalyticAngle}
Let~$f$ be a function satisfying Conditions~\textup{\ref{reg},~\ref{sum}}. Suppose that for any~$\eps$ in the interval~$[\eps',\eps''] \subset (0,\eps_{\infty})$ there is a point~$w(\eps)$ such that the foliation
\begin{equation*}
\Rt(-\infty,w(\eps))\cup\Ang(w(\eps)) \cup \Lt(w(\eps),\infty)
\end{equation*}
provides a Bellman candidate for~$f$ and~$\eps$ \textup(i.e. the function~$f$ falls under the scope of Proposition~\textup{\ref{AngleProp}}\textup). Then\textup, either the equation~$w(\eps) = z$ has only finite number of roots when~$\eps \in [\eps',\eps'']$ for any point~$z \in \mathbb{R}$\textup, or the angle is stable \textup($w(\eps)$ is constant when~$\eps \in [\eps',\eps'']$\textup).
\end{St}

\begin{proof}
The point~$u=w(\eps)$ is the root of the balance equation
\begin{equation*}
\Fr(u;-\infty;\eps) + \Fl(u;\infty;\eps) = 0.
\end{equation*} 
With the help of formulas~\eqref{RightForceInfinity} and~\eqref{LeftForceInfinity}, this equation can be rewritten as
\begin{equation*}
\int\limits_{\mathbb{R}}e^{\frac{-|t-u|}{\eps}}\,df''(t) = 0.
\end{equation*}
We note that the convolution on the left is an analytic function of~$\eps$ for any~$u$ fixed. So, if
\begin{equation*}
\Fr(z;-\infty;\eps) + \Fl(z;\infty;\eps) = 0
\end{equation*} 
infinitely many times on a finite interval, then the same equality holds for all~$\eps \in [\eps',\eps'']$, since an analytic function having infinitely many roots in a finite domain equals zero. 
\end{proof}

We note that an angle may visit a point infinitely many times if we consider infinite time. See the first example in Section~\ref{s54}. %We believe that Proposition~\ref{AnalyticAngle} is an exception, and the general situation is worse.
%\begin{Conj}\label{BirdieOscCConj}
%There exists a function~$f$ satisfying conditions~\textup{\eqref{reg},~\eqref{sum},} a decreasing sequence~$\{\eps_n\}$\textup,~$\eps_n \to \eps$\textup, and sequences~$\{w_n^{+}\}_n$\textup,~$\{a_n\}_n$\textup,~$\{b_n\}_n$\textup, and~$\{w_n^{-}\}_n$\textup,~$w_n^{-} < a_{2n} < b_{2n}$\textup,~$a_{2n+1} < b_{2n+1} < w_n^{+}$\textup, such that the Bellman function for~$f$ and~$\eps_{2n}$ has the foliation
%\begin{equation*}
%\Rt(-\infty,w_n^{-})\cup\Ang(w_n^{-})\cup\Lt(w_n^{-},a_{2n})\cup\LTroll(a_{2n},b_{2n})\cup\Ch([a_{2n},b_{2n}],[c_1,c_1])\cup\Lt(b_{2n},\infty),
%\end{equation*}
%whereas the Bellman function for~$f$ and~$\eps_{2n+1}$ has the foliation
%\begin{equation*}
%\Rt(-\infty,a_{2n+1})\cup\Ch([a_{2n+1},b_{2n+1}],[c_1,c_1]) \cup\RTroll(a_{2n+1},b_{2n+1})\cup\Rt(b_{2n+1},w_n^+) \cup\Ang(w_n^+)\cup\Lt(w_n^+,\infty).
%\end{equation*}
%\end{Conj}

\subsection{Boundary behavior}\label{s612}
As it was said in Subsection~\ref{s212}, Condition~\ref{sum} is only sufficient for the finiteness of the Bellman function~$\Bell$. It can be weakened slightly. We cite Theorem~$6.2$ from~\cite{SZ}.

\begin{Th}
If a measurable function~$f$ satisfies the condition
\begin{equation*}
\sum\limits_{k\in\mathbb{Z}}e^{-\frac{|k|}{\eps}}\!\!\!\sup\limits_{[\eps(k-2),\eps(k+2)]}\!\!\!|f| < \infty,
\end{equation*}
then the Bellman function~\textup{\eqref{Bf}} is finite.
\end{Th} 

There is a related question: when is the expression~$\int f(\varphi)$ well defined (and thus formula~\eqref{Bf} is relevant)? Both Condition~\ref{sum} and the theorem above provide conditions on~$|f|$. Maybe, there are some functions~$f$ oscillating at infinity such that~$\int |f(\varphi)|$ is infinite for some~$\varphi \in \BMO_{\eps}$, but the expression~$\int f(\varphi)$ can still be defined correctly? To study this question, we introduce yet another Bellman function:
\begin{equation}\label{Bff}
\Bellb(x_1,x_2;\,f) \;\df 
		\sup\big\{f[\varphi] \mid\; \av{\varphi}{I} = x_1,\av{\varphi^2}{I} = x_2,\;\varphi \in \BMO_{\eps}(I)\cap L_{\infty}(I)\big\}.
\end{equation} 
We note that it satisfies all the trivial properties of the function~$\Bell$ listed in Subsection~\ref{s211} and also Lemma~\ref{LMaj}. Moreover, it is well defined for any measurable function~$f$ that is locally bounded, whereas the function~$\Bell$ needs summability conditions such as Condition~\ref{sum} to be defined (and one also has to prove that the integral is well defined). In the case where~$\Bell$ is defined,~$\Bellb=\Bell$. A natural question arises: is the Bellman function~$\Bell$ well defined provided there exists a finite function~$G \in \Lambda_{\eps,f}$ (see formula~\eqref{Lambda})? Our aim here is to give an example of~$f$ for which the answer is negative. We need Proposition~$6.1$ from~\cite{SZ} (we formulate it in our particular case).

\begin{St}\label{Definitness}
Suppose that~$f$ is locally bounded from below and the minimal function~$\BG$ from~$\Lambda_{\eps,f}$ is finite. Then\textup, the integral~$\int f(\varphi)$ is well defined for all~$\varphi \in \BMO_{\eps}$ if and only if the function~$\Bell(\cdot\,;f_+)$ is finite, where $f_+=\max(f,0)$.
\end{St}

Namely, we will construct a function~$f$ and a Bellman candidate~$B$ in~$\Omega_1$ such that~$B$ is finite, but there exists a sequence of intervals~$\{\Delta_k\}_k$ tending to infinity,~$|\Delta_k| = \frac{1}{10}$,~$f(t) \geq e^t$ on~$\Delta_k$. Surely, for such a function~$f$,~$\Bell(\cdot\,;f_+)$ is infinite. Indeed, the value~$\int_{[0,1]} f_+(-\ln t)$ is infinite. So, by Proposition~\ref{Definitness}, there exists a function~$\varphi \in \BMO_{1}$ such that~$\int f(\varphi)$ is not well defined. It remains to prove the lemma below.

\begin{Le}
There exists a~$C^1$-smooth function~$f$\textup, a finite Bellman candidate~$B$ in~$\Omega_1$ for~$f$\textup, and a sequence of intervals~$\{\Delta_k\}_k$ tending to infinity such that~$|\Delta_k| = \frac{1}{10}$ and~$f(t) \geq e^t$ on~$\Delta_k$ for all~$k \in \mathbb{N}$.
\end{Le}
\begin{proof}
We begin with an abstract construction. Let~$v \in \mathbb{R}$, consider the domain~$\Lt(v,u)$, where~$u$ is very big. Suppose also that the values~$f(v)$,~$f'(v)$ and~$m(v)$ are given (as usual,~$m$ is the slope function given by formula~\eqref{linearity}). By~\eqref{difeq2},
\begin{equation*}
-m' + m = f',
\end{equation*} 
thus,~$m'(v)$ is also given. Let us set~$m''(t) = (e^{e^t})''= e^{e^t}(e^{2t} + e^t)\geq 0$ on this domain. In such a case, we can use the data and the Newton--Leibniz formula to find~$m'(t)$,~$m(t)$, and~$f(t)$, and build a locally concave (on~$\Lt(v,u)$) function~$B$ by formula~\eqref{linearity} with the help of Proposition~\ref{LeftTangentsCandidate}. It is clear that~$f$ is~$C^2$--smooth, and the functions~$f$ and~$m$ satisfy the inequalities (for sufficiently big~$t$)
\begin{equation}\label{Inequalities}
\begin{aligned}
1.1e^{e^t} \geq m(t) \geq 0.9e^{e^t};\\
f'(t) \geq -1.1e^t e^{e^t};\\
f(t) \geq -1.2e^{e^t}. 
\end{aligned}
\end{equation}
We set~$u$ to be so big that all these inequalities are valid at the point~$t = u$. After that, we choose some $w$, $w>u+3$, and extend the function~$B$ linearly (preserving the~$C^1$--smoothness) into the domain~$\MTC(\{[u,w]\})$, thus, defining the value of~$f$ on~$[u,w]$. Using~\eqref{Inequalities}, we see that~$f(u+2) = f(u) + 2m(u) \geq 0.6e^{e^u}$. 

It follows from linearity that~$f \geq 0.2e^{e^u}$ either on~$[u+1.9,u+2]$ or on~$[u+2,u+2.1]$. Indeed, the restriction of~$f$ to~$[u,w]$ is a quadratic polynomial. We know that~$f(u) \geq -1.2e^{e^u}$ and~$f(u+2) \geq 0.6e^{e^u}$. If one considers the two cases of positive and negative leading coefficient, he sees that~$f \geq 0.2e^{e^u}$ either on~$[u+1.9,u+2]$ or on~$[u+2,u+2.1]$. So, one of these two intervals is a good candidate to be one of the~$\Delta_k$ (since~$e^{e^u} \geq e^{u+2.1}$). It remains to extend the function~$B$ linearly to~$\Ang(w)$ and return to the left tangents.

Let us set the parameters~$f(0),m(0)$, and~$f'(0)$, and extend the function~$B$ linearly on the left (so,~$f$ is a quadratic polynomial there). To construct~$B$ on the right, we apply the procedure described above consecutively (i.e. setting~$v := 0$ first, then~$v := w$, and so on). 
\end{proof}

%\subsection{Other measures}\label{s613}

%\subsection{Duality theorem for continuous functions}\label{s614}

\section{Further development}\label{s62}
\subsection{More historical remarks}\label{s621}
As it was said in the introduction, the main ideas and results of the present text were known to the authors at the time of preparation of~\cite{5A}. There was a strong development in the field since that moment. We describe it briefly.

Several examples of Bellman functions given by formula~\eqref{Bf} for specific~$f$ played a significant role in the papers~\cite{LSSVZ,Osekowski2} (however, the second paper treats the case of very non-smooth~$f$). Though the theory from~\cite{5A} formally was not used, both papers admit inspiration by it. 

From the very beginning, it was clear that the method is not limited by the space~$\BMO$. Indeed, see the papers~\cite{BR,Rez,Va3}, where similar questions are studied on Muckenhoupt classes and Gehring (so called reverse H\"older) classes. All these particular cases were unified into a single extremal problem in~\cite{5AShortNew}. The authors also claim that all the constructions of the~$\BMO$ setting can be transferred to this more general one. It appears that one has to replace each notion (force, differentials of a chord, etc.) by its differential geometric analog. For example, the differentials can be expressed as an outer product of certain three vectors. Some hints to these differential geometric constructions may be found in~\cite{ISZ}. However, there are many technicalities to overcome that are not present in the~$\BMO$ case. That is why we decided first to present the full treatment of the~$\BMO$ case.

Theorem~\ref{MT} is not a miracle now. A relatively short and transparent proof of it (omitting the construction of the Bellman function) was given in~\cite{SZ} (in the general geometric setting of~\cite{5AShortNew}). The idea is that there is a third function (other than~$\Bell$ and the minimal locally concave~$\BG$) built as a solution of a certain optimization problem. The optimization problem is posed on the class of martingales starting from a point, wandering inside~$\Omega_{\eps}$, and ending their way on~$\FixedBoundary \Omega_{\eps}$. The value~$\BM(x)$ is the supremum of~$\E f(M)$ over all the martingales starting from the point~$x$. It is relatively easy to show that~$\BM = \BG$ (and this is a much more general fact). Then one shows that~$\BM = \Bell$ by proving two embedding theorems: each function from~$\BMO_{\eps}$ generates a martingale with ``the same'' final distribution, and vice versa, each martingale of the prescribed type generates a function from~$\BMO_{\eps}$.

We also mention that now one can work with non-quadratic semi-norms on~$\BMO$. Historically, the trick that allows to pass to~$p$-semi-norms, was invented by Slavin. Now it is written down in~\cite{Slavin2}, where the sharp constant for the John--Nirenberg inequality with respect to~$p$-semi-norm was found;~$1 \leq p \leq 2$ there (the case $p>2$ is considered in~\cite{SlVa4}). The trick was used in~\cite{LSSVZ} as well. The Bellman function that plays the major role in~\cite{Slavin2, SlVa4} is defined on the exponential strip and falls under the scope of the general setting in~\cite{5AShortNew}.

One can ask what happens if the underlying space on which the~$\BMO$ space is defined, has dimension~$2$ or greater. The most natural question is: if one defines the~$\BMO$ space on the cube~$Q \in \mathbb{R}^d$ as
\begin{equation*}
	\|\varphi\|_{\BMO(Q)} \!\!\df\; \Big(\sup_{J\subset Q}\av{|\varphi-\av{\varphi}{J}|^2}{J}\Big)^{\frac{1}{2}},
\end{equation*}
where~$J$ runs through all subcubes of~$Q$, what is the supremum of~$\lambda$'s such that~$e^{\lambda \frac{\varphi}{\|\varphi\|_{\BMO}}}$ is summable over~$Q$? It is not hard to see that~$\lambda \leq 1$. However, it is natural to conjecture that~$\lambda < 1$. Unfortunately, it is not clear how to find the optimal~$\lambda$. But one can solve the problem for dyadic classes\index{dyadic problems}.

%Let~$d \geq 1$ be the dimension, l
Let~$Q$ be a cube in~$\mathbb{R}^d$. By~$\mathcal{D}$ we denote the collection of all its dyadic subcubes. Define the~$\BMO^{\mathrm{dyad}}$-semi-norm by the formula
\begin{equation}\label{DyadicBMONorm}
\|\varphi\|_{\BMO^{\mathrm{dyad}}} \!\!\df\; \Big(\sup_{J\in\mathcal{D}(Q)}\av{|\varphi-\av{\varphi}{J}|^2}{J}\Big)^{\frac{1}{2}}.
\end{equation}  
Define the Bellman function by the formula~\eqref{Bf} with the usual~$\BMO$-norm replaced with~$\|\cdot\|_{\BMO^{\mathrm{dyad}}}$. The case~$f(t) = e^{\lambda t}$ (corresponding to the integral form of the John--Nirenberg inequality~\eqref{intJN}) was treated in~\cite{SlVa3}. It appeared that the Bellman function is the restriction of~$\boldsymbol{B}_{\eps'}(\cdot\,;\exp)$ to~$\Omega_{\eps}$, where~$\eps' > \eps$ is some explicit parameter (depending on~$\eps$ and~$d$). It would be also interesting to find sharp constants in the analogs of inequalities~\eqref{bmoequivnorms} and~\eqref{JN} for dyadic-type spaces. A more demanding task is to build a theory for the optimization problems on dyadic classes similar to the one presented here.

In Subsection~\ref{s224}, we said that the monotonic rearrangement operator is related to the optimization problem~\eqref{Bf}. Indeed, Theorem~\ref{MonotonicRearrangement} (from~\cite{Ivo}) helped us to guess the optimizers. There is a reverse influence. It was noticed in~\cite{SZ} that the martingales introduced there allow to prove sharp inequalities for the monotonic rearrangement operator on the class in question (e.g.~$\BMO$, Muckenhoupt classes, Gehring classes, etc.). The paper~\cite{SVZ} provides sharp estimates for the monotonic rearrangement operator from dyadic classes in arbitrary dimension to the corresponding continuous class on the interval.

\subsection{Conjectures and suggestions}\label{s622}
\paragraph{Other measures.} Let~$\mu$ be a Borel measure with finite variation on~$[0,1]$. We may consider a similar problem over this measure. Namely, consider the~$\BMO$ space with the seminorm~\eqref{BMOnorm2} where all averages are taken with respect to~$\mu$, i.e.
\begin{equation*}
\av{\varphi}{J} \df \frac{1}{\mu(J)}\int\limits_{J}\varphi(t)\,d\mu(t).
\end{equation*}
One may then consider the Bellman function given by formula~\eqref{Bf} where all averages are with respect to~$\mu$. It is easy to see that if the measure~$\mu$ does not contain atoms, then the resulting Bellman function is the same as before. It is interesting to see what happens in the other cases.

\paragraph{Other manifolds.} There are only two one-dimensional compact connected manifolds: a segment and a circle. We have studied the problem for the segment, but there is an absolutely similar setting on the circle. Namely, define the space~$\BMO^{\circ}$ of functions on~$\mathbb{T}$ by the seminorm
\begin{equation*}
	\|\varphi\|_{\BMO^{\circ}} \!\!\df\; \Big(\sup_{J\subset \mathbb{T}}\av{|\varphi-\av{\varphi}{J}|^2}{J}\Big)^{\frac{1}{2}},
\end{equation*}
the supremum is taken over all the arcs~$J \subset \mathbb{T}$.
Similarly, one can consider the Bellman function~$\Bell^{\circ}(x;f)$ given by formula~\eqref{Bf} with~$I$ replaced by~$\mathbb{T}$. It is clear that~$\Bell^{\circ} \leq \Bell$, because every function in~$\BMO^{\circ}$ can be identified with a function in~$\BMO(I)$. In some cases, this inequality may turn into equality. Anyway, it is interesting to find~$\Bell^{\circ}$ at least for some reasonable~$f$ (such as the exponential function).

\paragraph{Dyadic problems.}\index{dyadic problems}
Define the dyadic~$\BMO$ on the cube~$Q\subset \mathbb{R}^d$ by formula~\eqref{DyadicBMONorm} and consider the dyadic Bellman function 
\begin{equation}\label{BfDyad}
		\Belld(x_1,x_2;\,f) \;\df 
		\sup\big\{f[\varphi] \mid\; \av{\varphi}{Q} = x_1,\av{\varphi^2}{Q} = x_2,\;\varphi \in \BMO_{\eps}^{\mathrm{dyad}}(Q)\big\}.
	\end{equation} 
	It is easy to see that the domain of this function is~$\Omega_{\eps}$ and it satisfies the usual boundary conditions. As for the main inequality, one can easily prove that
	\begin{equation}\label{DyadicConcavity}
	\Belld(x) \geq 2^{-d}\sum\limits_{k=1}^{2^d}\Belld(x_k)\quad \hbox{provided}\quad x = 2^{-d}\sum\limits_{k=1}^{2^d}x_k,\quad x \in \Omega_{\eps}, \forall k\ x_k\in \Omega_{\eps}.
	\end{equation}
	In particular, the function~$\Belld$ is locally concave on~$\Omega_{\eps}$. However, condition~\eqref{DyadicConcavity} is much stronger. We recall a definition from~\cite{SZ}.
	\begin{Def}
	We call a domain~$\Omega$ an extension of~$\Omega_{\eps}$ if there exists an open convex unbounded set~$\Omega'$ such that~$\Omega = \{x \in\mathbb{R}^2\mid x_2 \geq x_1^2\} \setminus \Omega'$ and the closure of~$\Omega'$ lies in~$\{x \in\mathbb{R}^2\mid x_2 > x_1^2 + \eps^2\}$.
	\end{Def}
	\begin{Conj}\label{ExtensionConjecture}
	For every~$f$\textup,~$\eps$\textup, and~$d$ there exists an extension~$\Omega$ of~$\Omega_{\eps}$ such that
	\begin{equation*}
	\Belld(x) = \inf\Big\{G(x)\,\Big|\; G\,\hbox{is locally concave on}\;\Omega,\quad G(x_1,x_1^2) \geq f(x_1)\;\hbox{for all}\; x_1 \in \mathbb{R}\Big\},\quad x \in \Omega_{\eps}.
	\end{equation*}
	\end{Conj}
	This conjecture is verified for the case~$f(t) = e^t$ in the paper~\cite{SlVa3}. In the light of~\cite{5AShortNew}, Conjecture~\ref{ExtensionConjecture} opens the road towards a theory for dyadic Bellman functions similar to the one described in the present paper (however, the conjecture says nothing about how to find~$\Omega$).  
	
	One can pose a similar conjecture for the continuous~$\BMO$ on the cube of arbitrary dimension, however, up to the moment, there is a very little understanding of what happens there.
	
	\paragraph{Campanato spaces.}\index{Campanato spaces} The space~$\BMO$ can be thought of as a point on the scale of Morrey--Campanato spaces (see~\cite{KK} for the general theory of such spaces). Namely, consider the seminorm
	\begin{equation*}
	\|\varphi\|_{C_{2}^{\alpha,1}(I)} \!\!\df\; \Big(\sup_{J\subset I}|J|^{-\alpha}\av{|\varphi-\av{\varphi}{J}|^2}{J}\Big)^{\frac{1}{2}}.
	\end{equation*}
	Here~$\alpha \in (-\frac12,1]$. The space~$C_2^{\alpha,1}$ generated by this seminorm coincides with~$\BMO$ if~$\alpha=0$ and with the Lipschitz class if~$\alpha=1$. It seems reasonable to state a similar Bellman function problem on this space:
	\begin{equation*}
	B(x,w;f,\eps) = \sup\Big\{\av{f(\varphi)}{I}\,\Big|\; \av{\varphi}{I} =x_1,\av{\varphi^2}{I} = x_2, |I|=w, \|\varphi\|_{C_2^{\alpha,1}(I)} \leq \eps\Big\}.
	\end{equation*}
	One has to introduce the third variable~$w$ due to the scaling properties of the problem. Though it may seem questionable whether this function has good analytic properties, some hope comes from the paper~\cite{Osekowski4}, where the sharp equivalence between the Campanato and the classical seminorms is established for the Lipschitz class ($\alpha=1$).
